NeuTex: Neural Texture Mapping for Volumetric Neural Rendering

Recent work has demonstrated that volumetric scene representations combined with differentiable volume rendering can enable photo-realistic rendering for challenging scenes that mesh reconstruction fails on. However, these methods entangle geometry and appearance in a "black-box" volume that cannot be edited. Instead, we present an approach that explicitly disentangles geometry--represented as a continuous 3D volume--from appearance--represented as a continuous 2D texture map. We achieve this by introducing a 3D-to-2D texture mapping (or surface parameterization) network into volumetric representations. We constrain this texture mapping network using an additional 2D-to-3D inverse mapping network and a novel cycle consistency loss to make 3D surface points map to 2D texture points that map back to the original 3D points. We demonstrate that this representation can be reconstructed using only multi-view image supervision and generates high-quality rendering results. More importantly, by separating geometry and texture, we allow users to edit appearance by simply editing 2D texture maps.

==> tex/volume.tex <==
\subsection{Volume rendering}
Volumetric rendering is described by the following rendering equation.
\fanbo{a lot of details here}

\subsubsection{Radiance field}

The opacity of each point is given by
\[\alpha_t = 1-e^{\sigma l_t}\]
where $l_t$ is the light path length at point $t$ and $\sigma$ is the volumetric density.

The blending weight of a point is given by
\[w_t = \alpha_{t-1} + (1-\alpha_{t-1})\alpha_t \]
Finally the radiance at the camera is given by $L(c,\omega_o)$
\[\sum_{t=1}^m w_t L(x_t, \omega_o)\]

\subsubsection{Reflectance field}
\fanbo{a lot of details here}



\Comment{
\subsection{Overview}
Our method aims to disentangle the geometry (volumetric density) and appearance (object texture) in volumetric rendering, by storing the volumetric density in a MLP network $F_\sigma(x,y,z)$ which maps 3D coordinates to the volumetric density, and storing the appearance in another MLP network $F_{tex}(u,v, \mathbf{v})$ which takes texture-space coordinates $(u,v)$ and  the viewing direction $\mathbf{v}$ (parameterized by $\theta,\phi$) to predict an RGB radiance value. Next, we use a MLP network $F_{uv}(x,y,z)$ to associate any 3D coordinate with a 2D texture-space coordinate, indicating where to fetch colors for any 3D point. Next, we follow standard ray marching to accumulate point radiance along the camera ray to produce pixel colors.

To ensure that $F_{uv}$ maps 3D surfaces to a meaningful 2D texture space, we introduce another network $F^{-1}_{uv}$, which maps 2D UV coordinate back to 3D. We hope that this $F^{-1}_{uv}$ learns to map from texture-space coordinates back to object surfaces, essentially learning a parameterized representation of the object surfaces. Fig.~\ref{fig:arch} gives an illustration of our network architecture.

\subsection{Ray generation}
Given an training image with associated object mask, we sample $N$ pixels, 2/3 from foreground and 1/3 from the background. Next for each pixel, we compute a camera ray from its position and camera matrices. For each ray, we sample $M+2$ points on the ray, $(x_0,...,x_{M+1})$, starting from its first intersection with the unit cube $[-1,1]^3$; each consecutive points are separated by $2/M$ distance. Next we perturb the points along the ray within $0.1/M$ range; without such perturbation, the resulting image will contain aliased artifacts. We denote the current distance between the points $x_i$ and $x_{i+1}$ by $d_{i,i+1}$. Finally, we take the $M$ points in the middle $x_1,...,x_M$ as the shading points, with associated light path length $l_i = (d_{i-1,i} + d_{i,i+1}) / 2$.

\subsection{3D density network}
The 3D density network $F_\sigma$ takes a 3D coordinate $(x,y,z)\in\mathbb R^3$ (normalized to [-1,1] range) and outputs its volumetric density $\sigma\in\mathbb{R}_+$. To ensure the network represents high-frequency geometry details, we first apply positional encoding to the input $(x,y,z)$ similar to NeRF\cite{mildenhall2020nerf}, and then pass through a MLP to predict $\sigma$. 

Here we define the positional encoding function $\gamma: \mathbb{R}\to \mathbb{R}^{2k}$ with $k$ frequencies.
\[\gamma(t)_{2i-1} = \sin(2^i\pi t), \gamma(t)_{2i} = \cos(2^i\pi t), i=1,...,k\]
The input to the MLP is a concatenation of $(x,y,z)$ and the positional encodings of them, a vector of dimension $6k + 3$,
\[ [x \quad y \quad z \quad \gamma(x) \quad \gamma(y) \quad \gamma(z)] \]
In all our experiments, we set $k=10$.

\subsection{3D-2D UV network}
The 3D-2D UV network $F_{uv}$ determines where on the 2D texture to sample color for each 3D point $(x,y,z)$. Similar to AtlasNet\cite{groueix2018papier}, our 2D texture can be one or more texture maps with shape of squares of spheres. Since our experiments primarily focus on a single texture, we will introduce our networks in the case of single texture, but it can be extended to multiple texture maps as well. We model the 3D to 2D mapping with a MLP $F_{uv}$, whose input only consists of the point $(x,y,z)$. Positional encodings are not passed here as this network is supposed to smoothly map 3D space to 2D space without high-frequencies. The output of $F_{uv}$ depends on the shape of the texture: when using square texture, the output is a 2 dimensional texture coordinate $(u,v)\in [-1,1]^2$; when using sphere texture, to ensure the continuity of function $F_{uv}$, instead of 2 dimensional texture coordinate $(u,v)$, we predict 3 dimensional texture coordinate $(u,v,w)$ but normalize it to have unit 2-norm.

\subsection{2D texture network}
The 2D texture network $F_{tex}$ gives colors based on UV coordinates. For square textures, $F_{tex}$ takes $(u,v)$ and the unit viewing direction $\mathbf{v}$ as input and output a 3 channel color $\mathbf{L}$. Similar to the 3D density network, we take the concatenation of $u,v$, $\mathbf{v}$, and their positional encoding as input. For all our experiments, $u,v$ gets 10 positional encoding frequencies and $\mathbf{v}$ gets 6. After training, we can recover the view dependent texture by fixing a $\mathbf{v}$ and sample $F_{tex}$ with a uniform grid. We can also combine a standard texture sampler created 2D images with $F_{tex}$ to allow texture editing.

To handle sphere textures, we need a few modifications. First the input to $F_{tex}$ is changed to $(u,v,w)$ and $\mathbf{v}$ where $(u,v,w)$ is the unit vector indicating a point on the unit sphere. For texture editing, we also need to map the sphere to a 2D plane, and in this work, we choose to use a cube map as it gives small distortions.

\subsection{2D-3D inverse UV network}
The inverse UV network $F_{uv}^{-1}$ maps 2D coordinates (on a square or on a sphere) to 3D coordinates. It is modeled as a MLP that maps 2D input, either $(u,v)$ in a square texture or $(u,v,w)$ in a sphere texture, to a 3D point. $F_{uv}^{-1}$ can be considered as a parametric surface. We hope that after training, $F_{uv}^{-1}$ can represent the surface of the object.

\subsection{Rendering loss}
For each point $\mathbf{x} = (x,y,z)$ along a camera ray with direction $\mathbf{v}$, its radiance $\mathbf{L}$ is determined by the following computation,
\[u, v = F_{uv}(x,y,z)\]
\[\mathbf{L} = F_{tex}(u, v, \mathbf{v})\]
Recall the density of the point $\mathbf{x} = (x,y,z)$ is given by
\[\sigma = F_\sigma(x,y,z)\]
Next we use $t=1,...,M$ to index different points on a ray. $l_t$ is the light path length and $\mathbf{L}_t, \sigma_t$ is the radiance and density computed above.
\[\alpha_t = 1-e^{\sigma_t l_t}, \alpha_0 = 0\]
\[w_t = \alpha_{t-1} + (1-\alpha_{t-1})\alpha_t\]
\[\mathbf{L} = \sum_{t=1}^M w_t \mathbf{L}_t\]
Now the rendering loss is the L2 distance of predicted pixel value and ground truth pixel value.
\[L_{\mathrm{render}} = \frac{1}{N}\sum_{\mathrm{N\;rays}}||\mathbf{L}_{gt} - \mathbf{L}||_2^2\]

\subsection{UV Cycle loss}
To help learning a meaningful parameterized 2D surfaces $F_{uv}$, we introduce the UV cycle loss $L_{\text{cycle}}$ as follows. For each point $\mathbf{x}_t$ on a camera ray, 
\[\mathbf{x}_t' = F_{uv}^{-1}(F_{uv}(\mathbf{x}_t))\]
\[L_t = ||\mathbf{x}_t - \mathbf{x}_t'||_2^2\]
The $L$ here represents the distance from the original $\mathbf{x}_t$ after mapping to 2D with $F_{uv}$ and back to 3D with $F_{uv}^{-1}$. We hope that for all $\mathbf{x}_t$ near the object surface, $L_t$ is small, so $F_{uv}$ correctly finds the texture UV for $\mathbf{x}$ and $F_{uv}^{(-1)}$ gives the parameterized object surface. In volumetric rendering, object surface is characterized by high blending weight (opacity), so we will only apply this loss to input points with high blending weights. This is achieved by taking the weighted average of $L_t$ by blending weight $w_t$.
\[L_{\mathrm{cycle}} = \frac{1}{N}\sum_{\mathrm{N\; rays}} \sum_{t=1}^M w_t L_t\]
\fanbo{needs more explanation}

\subsection{Initialization}
We observe that the $F_{uv}^{-1}$ network has the same architecture as AtlasNet, and we get a point-cloud from COLMAP, so we may also supervise $F_{uv}^{-1}$ with this point cloud and Chamfer loss similar to AtlasNet. As shown in Fig.~\ref{fig:atlas}, the surface supervised from Chamfer loss is quite sensitive to noise, so we choose to use this surface as initialization of $F_{uv}^{-1}$.

\subsection{Training details}
For all our experiments, we use 256 uniformly sampled points along the rays. For each iteration, we sample 600 to 800 rays (depending on GPU memory usage) from an input image, 2/3 from the foreground and 1/3 from the background. We first train with Chamfer loss initialization together with rendering loss for 50,000 iterations. Next, we remove Chamfer loss and train with UV cycle loss and rendering loss until convergence after 500,000 iterations. Finally, we freeze $F_{\sigma}, F_{uv}$ and $F_{uv}^{-1}$ and only fine-tune the $F_{tex}$ network on fixed geometry until convergence. The whole process takes 2-3 days on a single RTX 2080Ti GPU. 
}
